ZCSD: a Computational Storage Device over Zoned Namespaces (ZNS) SSDs

The Big Data trend is putting strain on modern storage systems, which have to support high-performance I/O accesses for the large quantities of data. With the prevalent Von Neumann computing architecture, this data is constantly moved back and forth between the computing (i.e., CPU) and storage entities (DRAM, Non-Volatile Memory NVM storage). Hence, as the data volume grows, this constant data movement between the CPU and storage devices has emerged as a key performance bottleneck. To improve the situation, researchers have advocated to leverage computational storage devices (CSDs), which offer a programmable interface to run user-defined data processing operations close to the storage without excessive data movement, thus offering performance improvements. However, despite its potential, building CSD-aware applications remains a challenging task due to the lack of exploration and experimentation with the right API and abstraction. This is due to the limited accessibility to latest CSD/NVM devices, emerging device interfaces, and closed-source software internals of the devices. To remedy the situation, in this work we present an open-source CSD prototype over emerging NVMe Zoned Namespaces (ZNS) SSDs and an interface that can be used to explore application designs for CSD/NVM storage devices. In this paper we summarize the current state of the practice with CSD devices, make a case for designing a CSD prototype with the ZNS interface and eBPF (ZCSD), and present our initial findings. The prototype is available at https://github.com/Dantali0n/qemu-csd.

==> design.tex <==
\section{The Prototype}
We propose the design and implementation of ZCSD as a way to bridge the gap that we highlighted in the research landscape of Computational Storage Devices, where there is a lack of open-source, easily accessible prototypes for development and research. 

With this aim in mind, the design decisions for the device are centered around extensibility and programmability. The device is designed to allow users to experiment with APIs for a CSD and to program data-processing and management functionalities that can be offloaded to the storage device. Since the goal of the prototype is to enable research and exploration of CSD designs and APIs, these are the centerpiece design gials for the prototype:

\begin{enumerate}
	\item \textbf{extensibility}: The design must allow to extend the provided API and interface, enabling researchers to extend the current API. These can include new NVMe command sets or an extension to the API available to the BPF programs.
	
	\item \textbf{programmability}: It is important that the prototype can effectively be used for storage function programmability. The BPF programs that are loaded onto the CSD must be able to process and transfer data from a physical or virtual ZNS SSD to userspace.
	
	\item \textbf{observability}(?? trying to think of a better term): The goal of the prototype is not to provide a ready-made solution for CSD programmability, but rather to explore different offloading policies and mechanisms. As such, the prototype must facilitate the distinction between the data processing that happens on the host and the device, and should offer observability on the data transfers that happen to and from the device.
	
\end{enumerate}


ZCSD offers a lightweight and extensible interface that allows to experiment with CSD designs. The prototype provides an NVMe ZNS SSD device over SPDK (the device is emulated with QEMU), and allows to offload part of the computation to uBPF extensions (figure \ref{fig:prototypesteps}).

The design of the prototype does not constrain users for the offloading policies and functionalities, and rather allows to choose which data processing functionality to perform in the userspace application, what can be offloaded to the CSD device, either by extending the ZCSD device functionalities or by offloading user-specific uBPF extension. The choice of uBPF moreover allows to experiment with code extensions that are also compatible with kernel-space offloading, but leave the user with the freedom to change the programming language from uBPF to other user-space programming languages.


\textit{What can be developed with ZCSD:} the ZCSD prototype that we present in this paper was developed with extensibility in mind. To this day, there is still a lack of awareness as to what is the best offloading strategy for CSDs, and which API to use to exchange data. With ZCSD the user is not constrained by a specific design. Computation on data and storage function programmability can be implemented in the user application, hardcoded in the ZNS device or offloaded to a uBPF extension. Such flexibility is what allows to explore different design choices to evaluate the feasibility of CSD designs using a lightweight prototype and framework.

In the next section we will show initial experiments with the prototype, presenting an end-to end evaluation of the performance of the prototype, as well as a breakdown of the performance impact of the toolchain that we chose.


\begin{center}
	\begin{figure}
		\includegraphics[width=0.5\textwidth]{figures/zcsd-archslim.pdf}
		\caption{Overview of the components for the prototype}
		\label{fig:prototypesteps}
	\end{figure}
\end{center}





==> future-work.tex <==
\section{Future Work}
In this paper we presented an initial prototype for ZCSD. While the prototype is functional and allows to experiment with Computational Storage Device capabilities, its functionalities can be expanded to improve integration with existing systems, as well as improving the security of the data processing framework. In particular, we intend to focus on three main lines of work:
\begin{enumerate}
	\item integrate ZCSD with a file system for Flash storage like F2FS \cite{lee2015f2fs}
	\item support for additional, more advanced eBPF and uBPF verifiers
	\item built-in support for application-level data structures like hash tables and LSM trees for data processing insice ZCSD
\end{enumerate}
Such integrations and improvements will further improve the support for research experiments and more complex data processing workloads on the programmable storage device.
